Synthesizing Adversarial Negative Responses for Robust Response Ranking and Evaluation

Open-domain neural dialogue models have achieved high performance in response ranking and evaluation tasks. These tasks are formulated as a binary classification of responses given in a dialogue context, and models generally learn to make predictions based on context-response content similarity. However, over-reliance on content similarity makes the models less sensitive to the presence of inconsistencies, incorrect time expressions and other factors important for response appropriateness and coherence. We propose approaches for automatically creating adversarial negative training data to help ranking and evaluation models learn features beyond content similarity. We propose mask-and-fill and keyword-guided approaches that generate negative examples for training more robust dialogue systems. These generated adversarial responses have high content similarity with the contexts but are either incoherent, inappropriate or not fluent. Our approaches are fully data-driven and can be easily incorporated in existing models and datasets. Experiments on classification, ranking and evaluation tasks across multiple datasets demonstrate that our approaches outperform strong baselines in providing informative negative examples for training dialogue systems.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We test our approaches and baselines on two datasets for classification, dialogue ranking and evaluation tasks.

\subsection{Training Details}
We implemented our models using the PyTorch framework \cite{paszke2017automatic}. Initial base-uncased checkpoints for BERT~\cite{devlin-etal-2019-bert} and ELECTRA~\cite{Clark2020ELECTRAPT} are adapted from the huggingface transformers library~\cite{wolf-etal-2020-transformers}. All experiments are run on 4 NVIDIA 2080Ti GPUs. We trained the models with maximum sequence length of 128, batch size of 60 and using the Adam optimizer with an initial learning rate of 5e-5 with linear decay. For generation, we use temperature of 0.9, nucleus sampling with p equal to 0.9 and minimum length of 5. The maximum number of training epochs was set to 3 and the maximum sequence length was set to 128 tokens. 
We repeat each experiment five times with different random seeds, use the validation split to select the best model, and report the mean metric values.
% We used the validation set accuracy to select the best model for testing. 
Validation was done after every 200 batches.

\subsection{Experimental setup}
The primary dataset in our experiments is Dailydialog dataset~\cite{li-etal-2017-dailydialog}. We use the \textit{DailyDialog++} version open-sourced by~\cite{sai2020improving}. It consists of 16900 dialogue contexts in train set, 1028 in validation set and 1142 in the test set. Each context contains 5 positive and 5 adversarial negative responses collected by crowdsourcing, as well as 5 random responses. In the train set, only 9259 out of 16900 contexts have 5 adversarial negative responses. We conduct our experiments on the \textit{DailyDialog++} test set. We experiment on 3 tasks on this data - classification, ranking and evaluation. 
% The test contexts contain 5 positive, adversarial negative and random negative responses each. 
% The classification and ranking tasks are performed for both random negatives and adversarial negatives separately. 
For classification task, we report the accuracy metric following~\cite{sai2020improving}. The test set which contains 5 positive and 5 negative responses for each context.
For ranking task, the candidate set consists of one positive response along with either 5 random or 5 adversarial responses for each context. We report with standard ranking metrics - Recall $R_n@k$, mean reciprocal rank (MRR). Here $n=6$ as candidates consist of one positive response with 5 negative responses. 
For both classification and ranking tasks, we report results separately for the adversarial responses and the random negatives responses.

For dialogue evaluation task, we report the correlation of model scores with human provided ratings. We leverage the human ratings released by following sources - 1) 600 ratings for response ``sensibility'' from~\cite{zhao2020multi} with inter-rater agreement (Krippendorff’s $\alpha$ \cite{krippendorff2018content} $>$ 0.6). The responses consist of outputs from hierarchical recurrent encoder decoder (HRED) model with Attention~\cite{serban2016building} and Variational HRED model with attention. 2) 700 
ratings for response quality from~\cite{zhao-etal-2020-designing}. The responses are from 6 different generative models - Seq-2-Seq~\cite{NIPS2014_a14ac55a}, attentional Seq-2-Seq, HRED, VHRED, GPT2-small, and GPT2-medium~\cite{Wolf2019TransferTransfoAT} with greedy decoding, ancestral sampling, and nucleus sampling based decoding~\cite{holtzman2019curious}. The inter-rater agreement is high (Krippendorff’s $\alpha$ 0.815)  3) Since the first two sources do not cover retrieval model outputs, we additionally collect 100 response quality ratings for a retrieval model's (poly-encoder\cite{humeau2020poly}) selected responses and also for human written responses with moderate inter-annotator agreement (Cohen's Kappa 0.45~\cite{cohen1968weighted}). All data points belong to the Dailydialog dataset and ratings are scaled between 0-1. This brings the total to 1500 ratings for different context-response pairs.

The second dataset is PersonaChat dataset~\cite{zhang-etal-2018-personalizing}. It is
a corpus of human-human persona-conditioned conversations. It consists of 10,907 dialogs, with 8938 dialogues in the train set. We sample 2 random context-response pairs from each dialogue with a total of 17876 contexts for training. We evaluate various approaches on the ranking task on this dataset. 
% We also sample 1000 contexts for testing. 
There is no human-created adversarial test set available for PersonaChat dataset. To construct a PersonaChat adversarial test set, we randomly select an utterance from the dialog context and insert it in the set of candidate responses. This method of creating adversarial test set is inspired from~\citet{jia-liang-2017-adversarial} and \citet{whang2020response}. The adversarial candidate set of size n consists of the ground truth response, the utterance selected from the dialog context, and n-2 random negative responses. n is set to 10 for PersonaChat and R@1 is used to indicate R$_{10}$@1.

% \subsection{Evaluation Metrics}

\subsection{Baselines}

\noindent 
\textbf{Classification and Ranking} We compare the following approaches of creating adversarial negative response sets:

\noindent 
\textbf{Human}~\cite{sai2020improving} Human written adversarial responses. Annotators were instructed to create negative responses with high content similarity with the context.

\noindent 
\textbf{Random} Randomly sampled responses from other contexts.

\noindent
\textbf{Semi-hard}~\cite{li-etal-2019-sampling} Sampling scheme which selects samples from a batch based on their similarity scores, with a margin of $\alpha$ from the positive response score. We use Sentence-Bert~\cite{reimers-gurevych-2019-sentence} for semantic similarity calculation with $\alpha$ set to the recommended value of 0.07.

\noindent
\textbf{Token-subs}~\cite{kryscinski-etal-2020-evaluating} Training data is generated by applying a series of rule-based transformations on the positive responses. Transformations include pronoun, entity and number swapping, sentence negation and noise injection.

\noindent
\textbf{BM25} Top responses returned by BM25~\cite{DBLP:journals/ftir/RobertsonZ09} based on similarity with the context. Any ground truth response is removed from this response set if present by chance.
% the answer but match most context tokens. 
This baseline is inspired from~\cite{Karpukhin2020DensePR} and has shown strong performance for dense passage retrieval.
% Responses retrieved based on bm25 based similarity with the context.

\noindent 
\textbf{Mask-and-fill} (Ours) Our approach which infills utterances based conditioned on random contexts.

\noindent
\textbf{Key-context} (Ours) Our approach which generates responses conditioned on test context keywords and random context history.

\noindent
\textbf{Key-sem} (Ours) Our approach similar to key-context which additionally conditions on words semantically related to the keywords in context. 

For each dialogue context, 5 random negative responses were added to a set of 5 negative responses created from above approaches.


\noindent
\textbf{Models:} We experiment with the following model architectures in our experiments: 1) Bert~\cite{devlin-etal-2019-bert}. Specifically, we use the (SA-Bert)~\cite{10.1145/3340531.3412330} model, 2) Electra~\cite{Clark2020ELECTRAPT}, the model is pre-trained with a replaced token detection objective and employs a generator-discriminator framework, and 3) Poly-encoders~\cite{humeau2020poly}, the model allows for fast real-time inference by precomputing each candidate response representation once, and then ranking candidate responses for retrieval by attending to the context. 
% 4) ESIM~\cite{chen2019sequential}, the model encodes the context and response using a Bidirectional LSTM network, and then employs cross attention mechanism for response matching.


